Disce aut Deficere: Evaluating LLMs Proficiency on the INVALSI Italian Benchmark

Recent advancements in Large Language Models (LLMs) have significantly enhanced their ability to generate and manipulate human language, highlighting their potential across various applications. Evaluating LLMs in languages other than English is crucial for ensuring their linguistic versatility, cultural relevance, and applicability in diverse global contexts, thus broadening their usability and effectiveness. We tackle this challenge by introducing a structured benchmark using the INVALSI tests, a set of well-established assessments designed to measure educational competencies across Italy. Our study makes three primary contributions: Firstly, we adapt the INVALSI benchmark for automated LLM evaluation, which involves rigorous adaptation of the test format to suit automated processing while retaining the essence of the original tests. Secondly, we provide a detailed assessment of current LLMs, offering a crucial reference point for the academic community. Finally, we visually compare the performance of these models against human results. Additionally, researchers are invited to submit their models for ongoing evaluation, ensuring the benchmark remains a current and valuable resource.

==> tables/qualitative_examples_it.tex <==


\definecolor{lightblue}{rgb}{0.68, 0.85, 0.90}
\definecolor{lightgreen}{rgb}{0.68, 0.85, 0.45}
\definecolor{lightred}{rgb}{0.96, 0.68, 0.68}
\begin{table*}
\centering
\scriptsize
\begin{tabular}{|p{5cm}|p{5cm}|p{5cm}|}
\hline
\vspace{0.2cm}
\textbf{Original MC Question} \vspace{0.2cm}& \vspace{0.2cm}\textbf{Original MCC Question} \vspace{0.2cm}& \vspace{0.2cm}\textbf{Original RU Question} \vspace{0.2cm}
\\
\parbox{5cm}{Nella frase “Livia stava correndo nel parco, quando scoppiò un forte temporale” come sono gli eventi indicati dai due verbi?
\begin{itemize}
    \item Sono contemporanei e hanno la stessa durata
    \item Sono contemporanei e indicano azioni abituali
    \item Il primo evento interviene nel corso del secondo evento
    \item Il secondo evento interviene nel corso del primo evento
\end{itemize}} &
\parbox{5cm}{Leggi questa frase: “L’uccello notturno emise un suono talmente 
    acuto che fece molta paura agli abitanti del bosco”.\\
    Indica nella tabella quali parole sono nomi e quali non lo sono.\\ Metti 
    una crocetta per ogni riga della tabella.\\
\begin{itemize}
    \item L' -- È un nome / Non è un nome
    \item uccello -- È un nome / Non è un nome
    \item ...
\end{itemize}}
 &
\parbox{5cm}{Dove metteresti la lettera h? Se ci vuole, scrivila nel quadratino.\\
\\
\(\square\)avevo perso l’autobus così arrivai tardi \(\square\)a scuola.} \\
\hline
\vspace{0.2cm}
\textbf{Prompted MC Question} \vspace{0.2cm}& \vspace{0.2cm}\textbf{Prompted MCC Question} \vspace{0.2cm}& \vspace{0.2cm}\textbf{Prompted RU Question} \vspace{0.2cm} \\
\parbox{5cm}{\colorbox{yellow}{Domanda:} \\
Nella frase “Livia stava correndo nel parco, quando scoppiò un forte temporale” come sono gli eventi indicati dai due verbi? \\

\colorbox{yellow}{Opzioni:} 

['A. Sono contemporanei e hanno la stessa durata', \\'B. Sono contemporanei e indicano azioni abituali', \\'C. Il primo evento interviene nel corso del secondo evento', \\'D. Il secondo evento interviene nel corso del primo evento'] \\

\colorbox{yellow}{Istruzioni:} \\
\fcolorbox{yellow}{yellow}{\parbox{\dimexpr\linewidth-2\fboxsep-2\fboxrule}{Devi restituire la lettera corrispondente alla risposta esatta tra parentesi quadre.}} \\
\colorbox{yellow}{Formato della risposta: [lettera]} \\
\colorbox{yellow}{Risposta:} \vspace{0.2cm}}
 & \parbox{5cm}{\colorbox{yellow}{Domanda:} \\
Leggi questa frase: “L’uccello notturno emise un suono talmente acuto che fece molta paura agli abitanti del bosco”.\\

Indica se questa parola è un nome o no:\\
                L’ \\
                
\colorbox{yellow}{Opzioni:} 

['A. È un nome',\\ 'B. Non è un nome'] \\

\colorbox{yellow}{Istruzioni:} \\
\fcolorbox{yellow}{yellow}{\parbox{\dimexpr\linewidth-2\fboxsep-2\fboxrule}{Devi restituire la lettera corrispondente alla risposta esatta tra parentesi quadre.}} \\
\colorbox{yellow}{Formato della risposta: [lettera]} \\
\colorbox{yellow}{Risposta:} \vspace{0.2cm}} & 
\parbox{5cm}{\colorbox{yellow}{Domanda:} \\
 Dove metteresti la lettera h? Indica se è necessaria o meno a posto del **.\\

**avevo perso l’autobus così arrivai tardi a scuola. \\

\colorbox{yellow}{Opzioni:} 

['A. Necessaria',\\ 'B. Non necessaria'] \\

\colorbox{yellow}{Istruzioni:} \\
\fcolorbox{yellow}{yellow}{
\parbox{\dimexpr\linewidth-2\fboxsep-2\fboxrule}{Devi restituire la lettera corrispondente alla risposta esatta tra parentesi quadre.}} \\
\colorbox{yellow}{Formato della risposta: [lettera]} \\
\colorbox{yellow}{Risposta:} \vspace{0.2cm}} \\
\hline
\vspace{0.2cm}
\textbf{Model 1 Response}\vspace{0.2cm} & \vspace{0.2cm}
\textbf{Model 1 Response}\vspace{0.2cm} & \vspace{0.2cm}
\textbf{Model 1 Response}\vspace{0.2cm} \\

\colorbox{lightgreen}{[D]} \vspace{0.2cm} &
\colorbox{lightgreen}{[B. Non è un nome]} \vspace{0.2cm}&
\colorbox{lightgreen}{[B]} \vspace{0.2cm}\\

\hline
\vspace{0.2cm}
\textbf{Model 2 Response}\vspace{0.2cm} & \vspace{0.2cm}
\textbf{Model 2 Response}\vspace{0.2cm} & \vspace{0.2cm}
\textbf{Model 2 Response}\vspace{0.2cm} \\
\fcolorbox{lightred}{lightred}{\parbox{\dimexpr\linewidth-2\fboxsep-2\fboxrule}{[C. Il primo evento interviene nel corso del secondo evento]}}\vspace{0.2cm} &
\colorbox{lightgreen}{B. Non è un nome}\vspace{0.2cm} & \colorbox{lightred}{[A. Necessaria]}\vspace{0.2cm} \\
\hline
\end{tabular}
\caption{Examples of different types of questions in original Italian form and prompted format, along with correct and incorrect model answers.}
\label{tab:qualitative_examples_it}
\end{table*}




